Microwave spectroscopy of Q1D and Q2D organic conductors

This chapter reviews recent experimental studies of a novel open-orbit magnetic resonance phenomenon. The technique involves measurement of angle-dependent microwave magneto-conductivity and is, thus, closely related to the cyclotron resonance and angle-dependent magnetoresistance techniques. Data for three contrasting materials are presented: (TMTSF)2ClO4, alpha-(BEDT-TTF)2KHg(SCN)4 and kappa-(BEDT-TTF)2I3. These studies reveal important insights into the Fermiology of these novel materials, as well as providing access to important electronic parameters such as the in-plane Fermi velocity and quasiparticle scattering rate. It is argued that all three compounds exhibit coherent three-dimensional band transport at liquid helium temperatures, and that their low-energy magnetoelectrodynamic properties appear to be well explained on the basis of a conventional semiclassical Boltzmann approach. It is also suggested that this technique could be used to probe quasiparticles in nodal superconductors.

==> Hillref.tex <==
\begin{thebibliography}{100}

\bibitem{nesting}
A.~W. Overhauser, Phys. Rev. {\bf 128},  1437  (1962).

\bibitem{KagBook}
S. Kagoshima, H. Nagasawa, and T. Sambogni, {\em One-dimensional conductors}
  (Springer-Verlag, Berlin, 1988).

\bibitem{GrunerB}
G. Gr{\"u}ner, {\em Density Waves in Solids} (Addison Wesley, Reading, MA,
  1994).

\bibitem{IYS}
T. Ishiguro, K. Yamaji, and G. Saito, {\em Organic Superconductors} (Springer,
  Heidelberg, Germany, 1998).

\bibitem{Louati}
R. Louati, S. Charfi-Kaddour, A.~B. Ali, R. Bennaceur, and M. H{\'e}ritier,
  Phys. Rev. B {\bf 62},  5957  (2000).

\bibitem{Tanuma}
Y. Tanuma, K. Kuroki, Y. Tanaka, R. Arita, S. Kashiwaya, and H. Aoki, Phys.
  Rev. B {\bf 66},  094507  (2002).

\bibitem{Wosnitza}
J. Wosnitza, {\em Fermi Surfaces of Low-dimensional Organic Metals and
  Superconductors}, {\em Springer Tracts in Modern Physics} (Springer-Verlag,
  Berlin and Heidelberg, 1996).

\bibitem{JSReview}
J. Singleton, Rep. Prog. Phys. {\bf 63},  1111  (2000).

\bibitem{JSBook}
J. Singleton, {\em Band Theory and Electronic Properties of Solids} (Oxford
  University Press, Oxford, 2001).

\bibitem{KartsReview}
M.~V. Kartsovnik, Chem. Rev. {\bf 104},  5737  (2004).

\bibitem{Shoen}
D. Shoenberg, {\em Magnetic Oscillations in Metals} (Cambridge University
  press, Cambridge, 1984).

\bibitem{Abrikos}
A.~A. Abrikosov, {\em Fundamentals of the Theory of Metals} (Elsevier, New
  York, 1988).

\bibitem{Lebed86}
A.~G. Lebed, JETP Lett. {\bf 43},  174  (1986).

\bibitem{LebedBak}
A.~G. Lebed and P. Bak, Phys. Rev. Lett. {\bf 63},  1315  (1989).

\bibitem{gsbPRL90}
G.~S. Boebinger, G. Montambaux, M.~L. Kaplan, R.~C. Haddon, S.~V. Chichester,
  and L.~Y. Chiang, Phys. Rev. Lett. {\bf 64},  591  (1990).

\bibitem{OsadaPRL91}
T. Osada, A. Kawasumi, S. Kagoshima, N. Miura, and G. Saito, Phys. Rev. Lett.
  {\bf 66},  1525  (1991).

\bibitem{0onPRL91}
M.~J. Naughton, O.~H. Chung, M. Chaparala, X. Bu, and P. Coppens, Phys. Rev.
  Lett. {\bf 67},  3712  (1991).

\bibitem{OsadaPRL92}
T. Osada, S. Kagoshima, and N. Miura, Phys. Rev. B {\bf 46},  1812  (1992).

\bibitem{Karts93}
M.~V. Kartsovnik, A.~E. Kovalev, and N.~D. Kusch, J. Phys. I {\bf 3},  1187
  (1993).

\bibitem{DKC}
G.~M. Danner, W. Kang, and P.~M. Chaikin, Phys. Rev. Lett. {\bf 72},  3714
  (1994).

\bibitem{BlundPRB96}
S.~J. Blundell and J. Singleton, Phys. Rev. B {\bf 53},  5609  (1996).

\bibitem{Chash97}
E.~I. Chashechkina and P.~M. Chaikin, Phys. Rev. B {\bf 56},  13658  (1997).

\bibitem{Chash98}
E.~I. Chashechkina and P.~M. Chaikin, Phys. Rev. Lett. {\bf 80},  2181  (1998).

\bibitem{Lee98}
I.~J. Lee and M.~J. Naughton, Phys. Rev. B {\bf 58},  R13343  (1998).

\bibitem{KangSM03}
W. Kang, H. Kang, Y.~J. Jo, and S. Uji, Synth. Met. {\bf 133-134},  15  (2003).

\bibitem{LebedPRL04}
A.~G. Lebed, N.~N. Bagmet, and M.~J. Naughton, Phys. Rev. Lett. {\bf 93},
  157006  (2004).

\bibitem{YakovPRL06}
B.~K. Cooper and V.~M. Yakovenko, Phys. Rev. Lett. {\bf 96},  037001  (2006).

\bibitem{Zwick97}
F. Zwick, S. Brown, G. Margaritondo, C. Merlic, M. Onellion, J. Voit, and M.
  Grioni, Phys. Rev. Lett. {\bf 79},  3982  (1997).

\bibitem{Perel91}
A.~S. Perel, J.~S. Brooks, C.~J. G.~N. Langerak, T.~J. B.~M. Janssen, J.
  Singleton, J.~A. A.~J. Perenboom, and L.~Y. Chiang, Phys. Rev. Lett. {\bf
  67},  2072  (1991).

\bibitem{JSPRL92}
J. Singleton, F.~L. Pratt, M. Doporto, T.~J. B.~M. Janssen, M. Kurmoo, J.~A.
  A.~J. Perenboom, W. Hayes, and P. Day, Phys. Rev. Lett. {\bf 68},  2500
  (1992).

\bibitem{HillSM93}
S. Hill, J. Singleton, F.~L. Pratt, M. Doporto, W. Hayes, T.~J. B.~M. Janssen,
  J.~A. A.~J. Perenboom, M. Kurmoo, and P. Day, Synth. Met. {\bf 56},  2566
  (1993).

\bibitem{HillSM95}
S. Hill, A. Wittlin, J. van Bentum, J. Singleton, W. Hayes, J.~A. A.~J.
  Perenboom, M. Kurmoo, and P. Day, Synth. Met. {\bf 70},  821  (1995).

\bibitem{HillPRB96}
S. Hill, P.~S. Sandhu, M. Boonman, J.~A. A.~J. Perenboom, A. Wittlin, S. Uji,
  J.~S. Brooks, R. Kato, H. Sawa, and S. Aonuma, Phys. Rev. B {\bf 54},  13536
  (1996).

\bibitem{Poliskii}
A. Polisski, J. Singleton, P. Goy, W. Hayes, M. Kurmoo, and P. Day, J. Phys.
  Condens. Matter {\bf 8},  L195  (1996).

\bibitem{HillPRB97}
S. Hill, Phys. Rev. B {\bf 55},  4931  (1997).

\bibitem{BlundPRB97}
S.~J. Blundell, A. Ardavan, and J. Singleton, Phys. Rev. B {\bf 55},  R6129
  (1997).

\bibitem{OhtaSM97a}
H. Ohta, Y. Yamamoto, K. Akioka, M. Motokawa, T. Sasaki, and T. Fukase, Synth.
  Met. {\bf 86},  2011  (1997).

\bibitem{OhtaSM97b}
K. Akioka, H. Ohta, Y. Yamamoto, M. Motokawa, and K. Kanoda, Synth. Met. {\bf
  86},  2051  (1997).

\bibitem{OhtaSM97c}
H. Ohta, Y. Yamamoto, K. Akioka, M. Motokawa, and K. Kanoda, Synth. Met. {\bf
  86},  1913  (1997).

\bibitem{HillPB98}
S. Hill, J.~A. A.~J. Perenboom, T. Stalcup, N.~S. Dalal, T. Hathaway, and J.~S.
  Brooks, Physica B {\bf 246-247},  549  (1998).

\bibitem{ArdPRL98}
A. Ardavan, J.~M. Schrama, S.~J. Blundell, J. Singleton, W. Hayes, M. Kurmoo,
  P. Day, and P. Goy, Phys. Rev. Lett. {\bf 81},  713  (1998).

\bibitem{ArdPRB99}
A. Ardavan, S.~J. Blundell, and J. Singleton, Phys. Rev. B {\bf 60},  15500
  (1999).

\bibitem{Palassis}
C. Palassis, M. Mola, J. Tritz, S. Hill, S. Uji, K. Kawano, M. Tamura, T.
  Naito, and H. Kobayashi, Synth. Met. {\bf 120},  999  (2001).

\bibitem{OhtaSM99a}
Y. Oshima, N. Nakagawa, K. Akioka, H. Ohta, S. Okubo, M. Tamura, Y. Nishio, and
  K. Kajita, Synth. Met. {\bf 103},  1919  (1999).

\bibitem{OhtaSM99b}
H. Ohta, Y. Oshima, N. Nakagawa, K. Akioka, S. Okubo, and K. Kanoda, Synth.
  Met. {\bf 103},  1913  (1999).

\bibitem{OhtaSM01}
Y. Oshima, H. Ohta, S. Okubo, K. Koyama, M. Motokawa, M. Tamura, Y. Nishio, and
  K. Kajita, Synth. Met. {\bf 120},  853  (2001).

\bibitem{KovalevPRB02}
A.~E. Kovalev, S. Hill, and J.~S. Qualls, Phys. Rev. B {\bf 66},  134513
  (2002).

\bibitem{KovalevJAP03}
A. Kovalev, S. Hill, S. Takasaki, J. Yamada, and H. Anzai, J. Appl. Phys. {\bf
  93},  8665  (2003).

\bibitem{KovalevPRL03}
A.~E. Kovalev, S. Hill, K. Kawamo, M. Tamura, T. Naito, and H. Kobayashi, Phys.
  Rev. Lett. {\bf 91},  216402  (2003).

\bibitem{OhtaJPSJ02}
Y. Oshima, H. Ohta, K. Koyama, M. Motokawa, H.~M. Yamamoto, and R. Kato, J.
  Phys. Soc. Jpn. {\bf 71},  1031  (2002).

\bibitem{OhtaJPSJ03}
Y. Oshima, H. Ohta, K. Koyama, M. Motokawa, H. Yamamoto, R. Kato, M. Tamura, Y.
  Nishino, and K. Kajita, J. Phys. Soc. Jpn. {\bf 72},  143  (2003).

\bibitem{OhtaPRB03}
Y. Oshima, M. Kimata, K. Kishigi, H. Ohta, K. Koyama, M. Motokawa, and H.
  Nishikawa, Phys. Rev. B {\bf 68},  54526  (2003).

\bibitem{SusumuIJMP}
S. Takahashi, A.~E. Kovalev, S. Hill, S. Takasaki, J. Yamada, H. Anzai, J.~S.
  Qualls, K. Kawano, M. Tamura, T. Naito, and H. Kobayashi, Int. J. Mod. Phys.
  B {\bf 27-29},  3499  (2004).

\bibitem{SusumuJAP05}
S. Takahashi and S. Hill, J. Appl. Phys. {\bf 97},  10B106  (2005).

\bibitem{SusumuPRB05}
S. Takahashi, S. Hill, S. Takasaki, J. Yamada, and H. Anzai, Phys. Rev. B {\bf
  72},  024540  (2005).

\bibitem{MacKenzieRMP}
A.~P. MacKenzie and Y. Maeno, Rev. Mod. Phys. {\bf 75},  657  (2003).

\bibitem{HillPRL00}
S. Hill, J.~S. Brooks, Z.~Q. Mao, and Y. Maeno, Phys. Rev. Lett. {\bf 84},
  3374  (2000).

\bibitem{Hussey}
N.~E. Hussey, M. Abdel-Jawad, A. Carrington, A.~P. Mackenzie, and L. Balicas,
  Nature {\bf 425},  814  (2003).

\bibitem{ARPES}
A. Damasceli, Z. Hussain, and Z.-X. Shen, Rev. Mod. Phys. {\bf 75},  437
  (2003).

\bibitem{HillPRB00}
S. Hill, Phys. Rev. B {\bf 62},  8699  (2000).

\bibitem{CSCC}
D.~G. Clarke, S.~P. Strong, P.~M. Chaikin, and E.~I. Chashechkina, Science {\bf
  279},  2071  (1998).

\bibitem{WuPRL93}
W. Wu, I.~J. Lee, and P.~M. Chaikin, Phys. Rev. Lett. {\bf 91},  056601
  (2003).

\bibitem{WuPRL05}
W. Wu, P.~M. Chaikin, W. Kang, J. Shinagawa, W. Yu, and S.~E. Brown, Phys. Rev.
  Lett {\bf 94},  097004  (2005).

\bibitem{ChoiPRL05}
E.~S. Choi, J.~S. Brooks, H. Kang, Y.~J. Jo, and W. Kang, Phys. Rev. Lett. {\bf
  95},  187001  (2005).

\bibitem{Moses1}
P. Moses and R.~H. McKenzie, Phys. Rev. B {\bf 60},  7998  (1999).

\bibitem{Moses2}
R.~H. McKenzie and P. Moses, Phys. Rev. B {\bf 60},  11241  (1999).

\bibitem{Osadatc}
T. Osada, K. Kobayashi, and E. Ohmichi, Synth. Met. {\bf 135-136},  653
  (2003).

\bibitem{DressGrunBook}
M. Dressel and G. Gr{\"u}ner, {\em Electrodynamics Of Solids: Optical
  Properties Of Electrons In Matter} (Cambridge University Press, Cambridge,
  2002).

\bibitem{DressPRL96}
M. Dressel, A. Schwartz, G. Gr{\"u}ner, and L. Degiorgi, Phys. Rev. Lett. {\bf
  77},  398  (1996).

\bibitem{Red1}
O. Klein, S. Donovan, M. Dressel, and G. Gr{\"u}ner, Int. J. Infrared Millim.
  Waves {\bf 1993},  2423  (1993).

\bibitem{Red2}
S. Donovan, O. Klein, M. Dressel, K. Holczer, and G. Gr{\"u}ner, Int. J.
  Infrared Millim. Waves {\bf 14},  2459  (1993).

\bibitem{Red3}
M. Dressel, O. Klein, S. Donovan, and G. Gr{\"u}ner, Int. J. Infrared Millim.
  Waves {\bf 14},  2489  (1993).

\bibitem{MolaRSI}
M. Mola, S. Hill, P. Goy, and M. Gross, Rev. Sci. Inst. {\bf 71},  186  (2000).

\bibitem{SusumuRSI}
S. Takahashi and S. Hill, Rev. Sci. Inst. {\bf 76},  023114  (2005).

\bibitem{OsadaPB01}
T. Osada, H. Nose, and M. Karaguchi, Physica B {\bf 294-295},  402  (2001).

\bibitem{SusumuLT24}
S. Takahashi, S. Hill, S. Takasaki, J. Yamada, and H. Anzai, AIP conference
  proceedings {\bf 850},  619  (2006).

\bibitem{Mori90}
H. Mori, S. Tanaka, M. Oshima, G. Saito, T. Mori, Y. Maruyama, and H. Inokuchi,
  Bull. Chem. Soc. Jpn. {\bf 63},  2183  (1990).

\bibitem{Campos96}
C.~E. Campos, P.~S. Sandhu, J.~S. Brooks, and T. Ziman, Phys. Rev. B {\bf 53},
  12725  (1996).

\bibitem{NeilPRL99}
N. Harrison, Phys. Rev. Lett. {\bf 83},  1395  (1999).

\bibitem{NeilJPCM99}
N. Harrison, E. Rzepniewski, J. Singleton, P.~J. Gee, M.~M. Honold, P. Day, and
  M. Kurmoo, J. Phys.: Condens. Matter {\bf 11},  7227  (1999).

\bibitem{KovalevSSC94}
A. Kovalev, M. Kartsovnik, R. Shibaeva, L. Rozenberg, I. Schegolev, and N.
  Kushch, Solid State Commun. {\bf 89},  575  (1994).

\bibitem{Iye94}
Y. Iye, R. Yagi, N. Hanasaki, S. Kagoshima, H. Mori, H. Fujimoto, and G. Saito,
  J. Phys. Soc. Jpn. {\bf 63},  674  (1994).

\bibitem{Jason95}
J. Caulfield, S. Blundell, M. du~Croo~de Jongh, P. Hendriks, J. Singleton, M.
  Doporto, F. Pratt, A. House, J. Perenboom, W. Hayes, M. Kurmoo, and P. Day,
  Phys. Rev. B {\bf 51},  8325  (1995).

\bibitem{Hanasaki98}
N. Hanasaki, S. Kagoshima, T. Hasegawa, T. Osada, and N. Miura, Phys. Rev. B
  {\bf 57},  1336  (1998).

\bibitem{PeschPRB99}
V.~G. Peschansky and M.~V. Kartsovnik, Phys. Rev. B {\bf 60},  11207  (1999).

\bibitem{JSPRL02}
J.Singleton, P.~A. Goddard, A. Ardavan, N. Harrison, S.~J. Blundell, J.~A.
  Schlueter, and A.~M. Kini, Phys. Rev. Lett. {\bf 88},  037001  (2002).

\bibitem{Yamaji}
K. Yamaji, J. Phys. Soc. Jpn. {\bf 58},  1520  (1989).

\bibitem{Kobayashi95}
H. Kobayashi, K. Kawano, T. Naito, and A. Kobayashi, J. Mater. Chem. {\bf 5},
  1681  (1995).

\bibitem{Balthes}
E. Balthes, D. Schweitzer, I. Heinen, H.~J. Keller, W. Strunz, W. Biberacher,
  A.~G.~M. Jansen, and E. Steep, Z. Phys. B {\bf 99},  163  (1996).

\bibitem{RossScience}
R.~H. McKenzie, Science {\bf 278},  820  (1997).

\bibitem{TsueiRMP}
C.~C. Tsuei and J.~R. Kirtley, Rev. Mod. Phys. {\bf 72},  969  (2000).

\bibitem{Hosseini}
A. Hosseini, R. Harris, S. Kamal, P. Dosanjh, J. Preston, R. Liang, W.~N.
  Hardy, and D.~A. Bonn, Phys. Rev. B {\bf 60},  1349  (1999).

\bibitem{CorsonPRL00}
J. Corson, J. Orenstein, S. Oh, J. O'Donnell, and J.~N. Eckstein, Phys. Rev.
  Lett. {\bf 85},  2569  (2000).

\bibitem{TurnerPRL03}
P.~J. Turner, R. Harris, S. Kamal, M.~E. Hayden, D.~M. Broun, D.~C. Morgan, A.
  Hosseini, P. Dosanjh, G.~K. Mullins, J.~S. Preston, R. Liang, D.~A. Bonn, and
  W.~N. Hardy, Phys. Rev. Lett. {\bf 90},  237005  (2003).

\bibitem{Tamura91}
M. Tamura, H. Tajima, K. Yakushi, H. Kuroda, A. Kobayashi, R. Kato, and H.
  Kobayashi, J. Phys. Soc. Jpn. {\bf 60},  3861  (1991).

\bibitem{WosnitzaPRB02}
J. Wosnitza, J. Hagel, J.~S. Qualls, J.~S. Brooks, E. Balthes, D. Schweitzer,
  J.~A. Schlueter, U. Geiser, J. Mohtasham, R.~W. Winter, and G.~L. Gard, Phys.
  Rev. B {\bf 65},  180506  (2002).

\bibitem{Schwartz98}
A. Schwartz, M. Dressel, G. Gruner, V. Vescoli, L. Degiorgi, and T. Giamarchi,
  Phys. Rev. B {\bf 58},  1261  (1998).

\bibitem{DresselPRB05}
M. Dressel, K. Petukhov, B. Salameh, P. Zornoza, and T. Giamarchi, Phys. Rev. B
  {\bf 71},  075104  (2005).

\bibitem{DresselPRL03}
M. Dressel, N. Drichko, J. Schlueter, and J. Merino, Phys. Rev. Lett. {\bf 90},
   167002  (2003).

\bibitem{Ng}
H.~K. Ng, T. Timusk, and K. Bechgaard, J. Phys. Colloq. France {\bf 44},  867
  (1983).

\bibitem{CaoJPI96}
N. Cao, T. Timusk, and K. Bechgaard, J. Phys. I France {\bf 6},  1719  (1996).

\bibitem{Bech81}
K. Bechgaard, K. Carneiro, M. Olson, F.~B. Rasmussen, and C.~S. Jacobsen, Phys.
  Rev. Lett. {\bf 46},  852  (1981).

\bibitem{Donovan}
S. Donovan, Y. Kim, L. Degiorgi, M. Dressel, G. Gruner, and W. Wonneberger,
  Phys. Rev. B {\bf 49},  3363  (1994).

\end{thebibliography}

